Fast Training of Provably Robust Neural Networks by SingleProp

Recent works have developed several methods of defending neural networks against adversarial attacks with certified guarantees. However, these techniques can be computationally costly due to the use of certification during training. We develop a new regularizer that is both more efficient than existing certified defenses, requiring only one additional forward propagation through a network, and can be used to train networks with similar certified accuracy. Through experiments on MNIST and CIFAR-10 we demonstrate improvements in training speed and comparable certified accuracy compared to state-of-the-art certified defenses.

==> Tab/tab_added_baselines.tex <==
\begin{table}[htbp]
\centering
\adjustbox{max width = \textwidth}{
\begin{tabular}{llrrrrrr}
\toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
TRADES & \multirow{7}[1]{*}{$\epsilon=0.3$}          &   8264.6       &   \textbf{99.5 (0.7)\%}       &   0.0 (0.0)\%    &   0.0 (0.0)\%    &   0.0 (0.0)\%    &   0.0 (0.0)\%    \\
IBP    &          &   611.2       &     96.3 (1.7)\%     &  92.2 (2.5)\%     &  46.5 (5.1)\%     &  0.0 (0.0)\%     &  0.0 (0.0)\%     \\ 
IBP + $v$   &    &   589.6       &    90.1 (2.5)\%      &  88.9 (3.1)\%     &  86.5 (3.2)\%     &  \textbf{79.3 (3.7)\%}     &   59.0 (5.0)\%    \\ 
{$s$ only }  &     &   \textbf{273.3}       &    94.0 (2.1)\%      &   \textbf{92.7 (2.5)\%}    &   \textbf{90.1 (3.0)\%}    &   78.0 (3.9)\%    &  33.1 (4.7)\%     \\ 
\textbf{Double Margin} &  &  \cellcolor[rgb]{ .851,  .851,  .851}520.0        &    \cellcolor[rgb]{ .851,  .851,  .851}88.2 (2.6)\%      &  \cellcolor[rgb]{ .851,  .851,  .851} 86.7 (3.1)\%    &  \cellcolor[rgb]{ .851,  .851,  .851} 84.6 (3.4)\%    &  \cellcolor[rgb]{ .851,  .851,  .851}76.2 (3.9)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{61.9 (4.6)\%}     \\ 
IBP *     &       &  460.9      &     96.7 (1.4)\%     &  90.3 (2.6)\%     &  39.3 (4.6)\%     &  0.0 (0.0)\%     &  0.0 (0.0)\%     \\ 
\textbf{Double Margin} *  &   &  \cellcolor[rgb]{ .851,  .851,  .851} 415.3      &   \cellcolor[rgb]{ .851,  .851,  .851} 91.1 (2.6)\%      &   \cellcolor[rgb]{ .851,  .851,  .851}90.1 (2.9)\%    &\cellcolor[rgb]{ .851,  .851,  .851}  87.6 (3.2)\%     &   \cellcolor[rgb]{ .851,  .851,  .851}78.4 (3.9)\%    &  \cellcolor[rgb]{ .851,  .851,  .851} 60.4 (4.7)\%    \\ 
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
TRADES   & \multirow{5}[1]{*}{$\epsilon=8/255$}    &   56391.6       &    \textbf{62.2 (4.4)\%}     &  7.2 (2.5)\%    &  0.0 (0.0)\%     &  0.0 (0.0)\%    &   0.0 (0.0)\%   \\ 
IBP   &        &   2446.6       &    38.0 (4.2)\%      &  32.8 (4.0)\%     &  14.6 (3.1)\%     &   6.0 (2.2)\%    &   1.2 (0.8)\%    \\ 
IBP + $v$  &   &   3062.8       &   43.0 (4.6)\%       &  40.6 (4.2)\%     &  \textbf{34.2} (4.0)\%     &  27.0 (4.1)\%     &  18.2 (3.2)\%     \\ 
$s$ only &     &   \textbf{1475.8}       &     45.0 (5.1)\%     & \textbf{41.0 (3.8)\%}      &   33.8 (4.4)\%    &   22.8 (3.9)\%    &  10.4 (2.6)\%     \\
\textbf{Double Margin} &  & \cellcolor[rgb]{ .851,  .851,  .851}2198.7       & \cellcolor[rgb]{ .851,  .851,  .851}  43.2 (4.0)\%       & \cellcolor[rgb]{ .851,  .851,  .851}40.4 (4.6)\%      &\cellcolor[rgb]{ .851,  .851,  .851}  32.8 (4.4)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{28.6 (4.4)\%}     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{19.8 (3.5)\%}     \\
\midrule
\multicolumn{7}{c}{Pureconv CNN GTSRB, 4 layer} \\
    \midrule
MMR (4 epochs)   &  \multirow{5}[1]{*}{$\epsilon=8/255$} &    85377.2      &    \textbf{88.2 (2.8)\%}      &    53.6 (4.0)\%   &  18.2 (3.7)\%     &   4.2 (1.8)\%    &   0.0 (0.0)\%    \\ 
IBP & &  287.7       &  71.8 (3.9)\%        &  68.0 (4.3)\%     &  60.8 (4.3)\%     &  47.6 (4.7)\%     &  28.2 (3.5)\%     \\ 
 \textbf{Double Margin} & & \cellcolor[rgb]{ .851,  .851,  .851}283.1        &   \cellcolor[rgb]{ .851,  .851,  .851} 67.8 (4.4)\%      &  \cellcolor[rgb]{ .851,  .851,  .851}66.8 (4.3)\%     & \cellcolor[rgb]{ .851,  .851,  .851} 61.4 (4.3)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}56.4 (4.7)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{48.2 (4.5)\%}     \\ 
IBP *  &       &  266.6     &    78.0 (3.7)\%      &   \textbf{74.8 (3.7)\%}    &   62.2 (4.3)\%    &  45.6 (4.7)\%     &   26.8 (3.5)\%    \\ 
\textbf{Double Margin} * &  &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{258.1}      &    \cellcolor[rgb]{ .851,  .851,  .851} 75.6 (3.9)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}73.8 (4.2)\%      & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{65.0 (4.5)\%}     &  \cellcolor[rgb]{ .851,  .851,  .851} \textbf{57.2 (4.4)\%}    & \cellcolor[rgb]{ .851,  .851,  .851} 46.4 (4.4)\%     \\ 
\bottomrule
\end{tabular}}
\caption{CNN-Cert certified accuracies computed for 1000 points (MNIST) or 500 points (CIFAR/GTSRB) with std in ($\cdot$).
* denotes a different setting of regularization parameter $\lam$, decreased from $\frac{1}{2}$ to $\frac{1}{4}$. TRADES~\citep{zhang2019theoretically}, IBP ~\citep{gowal2019effectiveness}, MMR ~\citep{croce2019provable}. MMR is trained for 4 epochs due to its long training time.}
\label{tab:added_baselines}%
\end{table}

==> Tab/tab_cifar_relu.tex <==



%% CIFAR Relu full table:

\begin{table}[thbp]
    \vspace*{-0.2in}
  \centering
  \adjustbox{max width = \textwidth}{
       \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
    Normal &       & 141.1 & 61.5\% & 22.0\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 1062.8 & 58.0\% & 24.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{5}[2]{*}{$\epsilon=2/255$} & 51203.7 & 57.5\% & 24.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 22351.6 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 394.8 & 47.0\% & 37.5\% & 22.0\% & 3.5\% & 3.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 409.4 & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{394.5} & \cellcolor[rgb]{ .851,  .851,  .851}45.0\% & \cellcolor[rgb]{ .851,  .851,  .851}40.0\% & \cellcolor[rgb]{ .851,  .851,  .851}34.0\% & \cellcolor[rgb]{ .851,  .851,  .851}25.5\% & \cellcolor[rgb]{ .851,  .851,  .851}24.0\% & \cellcolor[rgb]{ .851,  .851,  .851}2.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% \\
    \midrule
    Adv. Training & \multirow{5}[2]{*}{$\epsilon=8/255$} & 51893.6 & \textbf{60.5\%} & 25.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 21918.7 & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 3.5\% & 3.5\% & 3.5\% \\
    IBP   &       & 410.0 & 37.5\% & 35.0\% & 32.5\% & 20.0\% & 17.5\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 396.1 & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}409.7 & \cellcolor[rgb]{ .851,  .851,  .851}45.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{45.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{43.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{40.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{39.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{28.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{22.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{19.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{15.0\%} \\
    \midrule
    \multicolumn{12}{c}{Pooling CNN CIFAR, 5 layer} \\
    \midrule
    Normal &       & 1164.9 & 65.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 828.8 & 59.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=8/255$} & 4015.1 & 43.0\% & 15.5\% & 8.5\% & 3.0\% & 3.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{1676.9} & \textbf{58.5\%} & 8.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}2899.5 & \cellcolor[rgb]{ .851,  .851,  .851}40.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{32.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{30.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{24.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{23.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{5.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%}& \cellcolor[rgb]{ .851,  .851,  .851}\textbf{0.5\%} \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies on CIFAR networks}
    \label{tab:cifar_relu}
    \vspace*{-0.2in}
  %
\end{table}%

==> Tab/tab_cifar_tanh.tex <==


%% Cifar tanh table

\begin{table}[htbp]
  \centering
    \begin{tabular}{rlrrrrrrrrrr}
    \toprule
    \multicolumn{1}{l}{Network} & Method & \multicolumn{1}{l}{Runtime} & \multicolumn{1}{l}{$\epsilon=0$} &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Small CNN CIFAR} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Bounded $\epsilon = 2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = 8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Bounded $\epsilon = 8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Medium CNN CIFAR} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = 2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = 8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Large CNN CIFAR} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Pooling CNN CIFAR} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Resnet CNN CIFAR} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =2/255$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =8/255$ &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    \caption{CIFAR Tanh Table}
  %
\end{table}%

==> Tab/tab_full.tex <==


\begin{table}[htbp]
\centering
\adjustbox{max width = 0.9\textwidth}{
\begin{tabular}{llrrrrrr}
\toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_\infty$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{88.0\%} & \textbf{81.0\%} & \textbf{63.5\%}\\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7 & 68.5\% & 59.5\% & 50.5\% & 9.0\% & 0.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 76.0\% & 57.5\% & 4.0\% & 0.0\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.25$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.50$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.75$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_1$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 & \textbf{89.0\%} & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7 & 68.5\% & \textbf{62.5\%} & \textbf{53.0\%} & \textbf{35.5\%} & \textbf{11.0\%} \\ 
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$4.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_0$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 &  \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 85.5\% & 84.0\% & 82.0\% & 60.5\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_\infty$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$  & 3058.8 & \textbf{42.5\%} & \textbf{40.0\%} & \textbf{35.0\%} & \textbf{31.0\%} & \textbf{20.5\%} \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4  & 30.0\% & 28.5\% & 24.5\% & 20.5\% & 19.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  2991.7 & 28.0\% & 27.0\% & 25.0\% & 22.5\% & 19.5\% \\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.15$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_1$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$ & 3058.8  & \textbf{42.5\%} & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4  & 30.0\% & \textbf{28.5\%} & \textbf{27.0\%} & \textbf{23.5\%} & \textbf{22.5\%}\\ 
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$4.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_0$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$ & 3058.8  & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  2991.7 & 28.0\% & 27.5\% & 27.5\% & 26.0\% & 24.0\% \\
\bottomrule
\vspace{6mm}
\end{tabular}}
\caption{CNN-Cert certified accuracies for \textbf{Effectiveness on other norms}}
\label{tab:lp_norm_main}%
\end{table}

\begin{table}[htbp]
  \centering
  \adjustbox{max width = \textwidth}{
    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
    \textbf{Double Margin} & \multirow{2}[2]{*}{$\epsilon=0.2$} & 521.1 & \textbf{95.5\%} & \textbf{95.5\%} & 95.2\% & 94.2\% & 93.5\% & 91.7\% & 81.3\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin Ensemble} &       & 1411.2 & \textbf{95.5\%} & \textbf{95.5\%} & \textbf{95.5\%} & \textbf{95.5\%} & \textbf{94.5\%} & \textbf{93.5\%} & \textbf{85.5\%} & 0.0\% & 0.0\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
    \textbf{Double Margin} & \multirow{2}[2]{*}{$\epsilon=8/255$} & 2517.3 & 42.8\% & 41.8\% & 39.8\% & 36.8\% & 36.3\% & 26.8\% & 18.8\% & 15.8\% & \textbf{13.8\%} \\
    \textbf{Double Margin Ensemble} &       & 6566.2 & \textbf{46.0\%} & \textbf{44.0\%} & \textbf{43.5\%} & \textbf{40.0\%} & \textbf{38.0\%} & \textbf{27.0\%} & \textbf{22.0\%} & \textbf{16.0\%} & 11.0\% \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert accuracies for \textbf{Model ensemble}. The ensemble uses three models with different random initialization and random training batches. For fair comparison with standard Double Margin, three models with the same random initializations and training batches are trained independently. The training times and certified accuracies for standard Double Margin are averaged over these three models.}
  \label{tab:ensemble}%
\end{table}%



\begin{table}[htbp]
  \centering
  \adjustbox{max width = \textwidth}{
    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Pureconv CNN GTSRB, 4 layer} \\
    \midrule
    Normal &       & 119.6 & 92.0\% & 77.5\% & 57.5\% & 37.0\% & 35.0\% & 6.5\% & 1.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=2/255$} & 289.3 & \textbf{84.0\%} & \textbf{81.5\%} & \textbf{78.0\%} & 65.0\% & 63.5\% & 31.0\% & 14.5\% & 10.0\% & 5.5\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{282.6} & \cellcolor[rgb]{ .851,  .851,  .851}83.0\% & \cellcolor[rgb]{ .851,  .851,  .851}80.0\% & \cellcolor[rgb]{ .851,  .851,  .851}77.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{68.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{67.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}43.5\% & \cellcolor[rgb]{ .851,  .851,  .851}27.5\% & \cellcolor[rgb]{ .851,  .851,  .851}22.0\% & \cellcolor[rgb]{ .851,  .851,  .851}16.5\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=8/255$} & 287.7 & 64.0\% & 63.0\% & 62.0\% & 58.5\% & 57.0\% & 44.5\% & 31.5\% & 26.0\% & 22.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}283.1 & \cellcolor[rgb]{ .851,  .851,  .851}68.0\% & \cellcolor[rgb]{ .851,  .851,  .851}67.5\% & \cellcolor[rgb]{ .851,  .851,  .851}67.0\% & \cellcolor[rgb]{ .851,  .851,  .851}65.0\% & \cellcolor[rgb]{ .851,  .851,  .851}64.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{58.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{52.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{50.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{45.5\%} \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies on GTSRB networks.}
  \label{tab:gtsrb}%
\end{table}%



\begin{table}[htbp]
\centering
\adjustbox{max width = 0.72\textwidth}{
\begin{tabular}{llrrrrrr}
\toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_\infty$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{88.0\%} & \textbf{81.0\%} & \textbf{63.5\%}\\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=1$  & 592.0  & 68.5\% & 61.5\% & 50.0\% & 22.5\% & 1.5\%\\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7 & 68.5\% & 59.5\% & 50.5\% & 9.0\% & 0.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 76.0\% & 57.5\% & 4.0\% & 0.0\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.25$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.50$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.75$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_2$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$ & 609.7 & \textbf{89.0\%} & \textbf{84.5\%} & 0.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=1$  & 592.0  & 68.5\% & 62.0\% & \textbf{52.0\%} & \textbf{41.5\%} & \textbf{24.0\%}\\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7  & 68.5\% & 61.0\% & 51.5\% & 34.0\% & 9.0\%\\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 80.5\% & 69.0\% & 39.0\% & 7.5\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$4.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_1$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 & \textbf{89.0\%} & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=1$  & 592.0 & 68.5\% & 60.5\% & 39.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7 & 68.5\% & \textbf{62.5\%} & \textbf{53.0\%} & \textbf{35.5\%} & \textbf{11.0\%} \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 81.0\% & 69.0\% & 39.5\% & 6.5\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$4.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer, $\ell_0$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=0.3$  & 609.7 &  \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} & \textbf{89.0\%} \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=1$  & 592.0 & 68.5\% & 68.5\% & 68.5\% & 68.5\% & 68.5\%\\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=4$  & 593.7 &  68.5\% & 68.5\% & 68.5\% & 68.5\% & 67.5\%\\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  593.3 & 86.0\% & 85.5\% & 84.0\% & 82.0\% & 60.5\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_\infty$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$  & 3058.8 & \textbf{42.5\%} & \textbf{40.0\%} & \textbf{35.0\%} & \textbf{31.0\%} & \textbf{20.5\%} \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=0.2$  & 2969.9 & 35.0\% & 32.5\% & 27.5\% & 25.5\% & 17.5\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4  & 30.0\% & 28.5\% & 24.5\% & 20.5\% & 19.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  2991.7 & 28.0\% & 27.0\% & 25.0\% & 22.5\% & 19.5\% \\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.15$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_2$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$ & 3058.8 & \textbf{42.5\%} &  \textbf{33.5\%} & 18.5\% & 3.5\% & 0.0\%\\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=0.2$  & 2969.9 & 35.0\% & 33.0\% & \textbf{31.5\%} & \textbf{28.0\%} & \textbf{26.5\%}  \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4 & 30.0\% & 28.5\% & 27.0\% & 26.0\% & 23.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  & 2991.7 & 28.0\% & 27.0\% & 26.5\% & 25.0\% & 24.0\%\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.50$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.50$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_1$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$ & 3058.8  & \textbf{42.5\%} & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=0.2$  & 2969.9 & 35.0\% & \textbf{31.5\%} & \textbf{28.0\%} & \textbf{24.0\%} & 20.0\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4  & 30.0\% & 28.5\% & 27.0\% & 23.5\% & 22.5\%\\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  2991.7 & 28.0\% & 27.5\% & 26.0\% & \textbf{24.0\%} & \textbf{23.5\%}\\
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1.00$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$2.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3.00$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$4.00$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer, $\ell_0$} \\
    \midrule
\textbf{Double Margin} $\ell_\infty$  &  $\eps=8/255$ & 3058.8  & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} & \textbf{42.5\%} \\ 
\textbf{Double Margin} $\ell_2$  &  $\eps=0.2$  & 2969.9 & 35.0\% & 35.0\% & 35.0\% & 34.5\% & 34.0\% \\ 
\textbf{Double Margin} $\ell_1$  &  $\eps=2$  & 2975.4 & 30.0\% & 30.0\% & 30.0\% & 29.0\% & 27.5\% \\ 
\textbf{Double Margin} $\ell_0$  &  $\eps=2$  &  2991.7 & 28.0\% & 27.5\% & 27.5\% & 26.0\% & 24.0\% \\
\bottomrule
\end{tabular}}
\caption{CNN-Cert certified accuracies for various $\ell_p$ versions of Double Margin computed for different $\ell_p$ perturbation sizes.}
\label{tab:lp_norm}%
\end{table}



\begin{table}[htbp]
  \centering
   \adjustbox{max width = 0.85\textwidth}{
            \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
    Normal &       & 185.7 & 98.5\% & 9.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 626.3 & 99.5\% & 81.0\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.1$} & 8873.6 & \textbf{100.0\%} & 97.0\% & 91.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27994.8 & 48.5\% & 48.5\% & 48.5\% & 48.5\% & 48.0\% & 48.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 613.1 & 99.5\% & \textbf{99.5\%} & \textbf{99.0\%} & \textbf{98.0\%} & \textbf{96.5\%} & 83.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 602.3 & 97.5\% & 89.5\% & 40.5\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 686.7 & 98.0\% & 90.0\% & 34.5\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9710.9 & 98.5\% & 96.5\% & 92.0\% & 84.5\% & 75.0\% & 54.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}520.0 & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.0\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{96.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textbf{Double Margin +L1} &       & \cellcolor[rgb]{ .851,  .851,  .851}545.5 & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{96.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{95.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.2$} & 8786.8 & 99.0\% & 98.5\% & 91.0\% & 38.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27999.5 & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 75.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 614.0 & 97.5\% & 97.5\% & 97.0\% & 96.5\% & 96.0\% & 78.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 592.6 & 95.0\% & 90.0\% & 59.0\% & 12.5\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 684.8 & 95.0\% & 89.5\% & 55.5\% & 10.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9669.4 & 93.0\% & 92.0\% & 86.5\% & 80.0\% & 63.5\% & 46.0\% & 3.5\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{518.8} & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.0\% & \cellcolor[rgb]{ .851,  .851,  .851}93.0\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}81.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textbf{Double Margin +L1} &       & \cellcolor[rgb]{ .851,  .851,  .851}546.1 & \cellcolor[rgb]{ .851,  .851,  .851}95.5\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}93.5\% & \cellcolor[rgb]{ .851,  .851,  .851}82.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.3$} & 8760.5 & 99.5\% & 98.5\% & 91.5\% & 38.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27966.8 & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 29.5\% & 28.5\% & 25.0\% & 0.0\% \\
    IBP   &       & 611.2 & 95.5\% & 95.5\% & 95.5\% & 90.5\% & 76.5\% & 39.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 595.8 & 94.0\% & 90.0\% & 65.0\% & 23.0\% & 5.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 686.5 & 95.0\% & 88.0\% & 53.5\% & 13.5\% & 3.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9657.1 & 90.0\% & 86.5\% & 70.5\% & 55.0\% & 30.5\% & 13.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}520.0 & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.0\% & \cellcolor[rgb]{ .851,  .851,  .851}88.5\% & \cellcolor[rgb]{ .851,  .851,  .851}88.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}86.5\% & \cellcolor[rgb]{ .851,  .851,  .851}80.0\% & \cellcolor[rgb]{ .851,  .851,  .851}66.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textbf{Double Margin +L1} &       & \cellcolor[rgb]{ .851,  .851,  .851}547.1 & \cellcolor[rgb]{ .851,  .851,  .851}91.0\% & \cellcolor[rgb]{ .851,  .851,  .851}90.5\% & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.5\% & \cellcolor[rgb]{ .851,  .851,  .851}89.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{83.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{68.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{12}{c}{Medium CNN MNIST, 7 layer} \\
    \midrule
    Normal &       & 387.4 & 100\% & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\%   & 0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=0.1$} & 1553.6 & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & 90\%  & 85\%  & 0\%   & 0\%   & 0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1360.4} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}0\% & \cellcolor[rgb]{ .851,  .851,  .851}0\% & \cellcolor[rgb]{ .851,  .851,  .851}0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=0.2$} & 1553.2 & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & 95\%  & 80\%  & 40\%  & 0\%   & 0\%   & 0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1360.6 & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{100\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{90\%} & \cellcolor[rgb]{ .851,  .851,  .851}0\% & \cellcolor[rgb]{ .851,  .851,  .851}0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=0.3$} & 1550.6 & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & 90\%  & 50\%  & 0\%   & 0\%   & 0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1362.3 & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}90\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{90\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{80\%} & \cellcolor[rgb]{ .851,  .851,  .851}0\% \\
    \midrule
    \multicolumn{12}{c}{Pooling CNN MNIST, 5 layer} \\
    \midrule
    Normal &       & 226.0 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 145.1 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[1]{*}{$\epsilon=0.1$} & 7747.8 & \textbf{99.5\%} & \textbf{98.5\%} & 4.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 1075.6 & 98.0\% & 92.0\% & 77.5\% & 64.5\% & 40.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 337.3 & 98.5\% & 87.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1070.3 & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}86.0\% & \cellcolor[rgb]{ .851,  .851,  .851}80.0\% & \cellcolor[rgb]{ .851,  .851,  .851}73.0\% & \cellcolor[rgb]{ .851,  .851,  .851}55.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.2$} & 7573.4 & \textbf{99.5\%} & \textbf{98.5\%} & 16.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 1082.8 & 96.0\% & 78.0\% & 63.5\% & 51.0\% & 39.0\% & 20.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{336.7} & 97.0\% & 90.0\% & 4.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}680.5 & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{93.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{91.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{89.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{82.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}4.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.3$} & 7518.9 & \textbf{99.5\%} & 97.5\% & 23.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 395.4 & 95.0\% & 76.5\% & 56.0\% & 44.0\% & 33.5\% & 13.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 337.5 & 97.0\% & 88.5\% & 13.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}408.0 & \cellcolor[rgb]{ .851,  .851,  .851}88.0\% & \cellcolor[rgb]{ .851,  .851,  .851}88.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}86.5\% & \cellcolor[rgb]{ .851,  .851,  .851}85.0\% & \cellcolor[rgb]{ .851,  .851,  .851}81.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{43.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{0.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{12}{c}{1-Resnet CNN MNIST, 4 layer} \\
    \midrule
    Normal &       & 210.1 & 98.5\% & 2.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 145.1 & 99.0\% & 51.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.1$} & 7705.8 & \textbf{99.0\%} & 97.5\% & 93.5\% & 22.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 600.2 & \textbf{99.0\%} & 95.5\% & 94.5\% & 90.5\% & 87.5\% & 81.0\% & 3.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 318.4 & 93.0\% & 85.5\% & 58.5\% & 25.5\% & 9.0\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}629.3 & \cellcolor[rgb]{ .851,  .851,  .851}98.0\% & \cellcolor[rgb]{ .851,  .851,  .851}80.5\% & \cellcolor[rgb]{ .851,  .851,  .851}77.0\% & \cellcolor[rgb]{ .851,  .851,  .851}74.5\% & \cellcolor[rgb]{ .851,  .851,  .851}70.0\% & \cellcolor[rgb]{ .851,  .851,  .851}65.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.2$} & 7554.4 & 98.0\% & \textbf{98.0\%} & \textbf{95.0\%} & 69.0\% & 9.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 593.3 & 97.5\% & 62.0\% & 57.0\% & 52.0\% & 50.0\% & 45.0\% & 10.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{317.8} & 93.0\% & 85.5\% & 67.0\% & 34.5\% & 17.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}630.0 & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}52.0\% & \cellcolor[rgb]{ .851,  .851,  .851}51.5\% & \cellcolor[rgb]{ .851,  .851,  .851}50.5\% & \cellcolor[rgb]{ .851,  .851,  .851}50.0\% & \cellcolor[rgb]{ .851,  .851,  .851}46.0\% & \cellcolor[rgb]{ .851,  .851,  .851}28.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.3$} & 7583.4 & \textbf{99.0\%} & 97.5\% & 94.5\% & 73.0\% & 17.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 600.3 & 96.5\% & 73.5\% & 69.0\% & 63.5\% & 57.5\% & 51.0\% & 13.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 319.0 & 93.0\% & 86.0\% & 70.5\% & 40.0\% & 19.5\% & 4.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}630.4 & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}77.0\% & \cellcolor[rgb]{ .851,  .851,  .851}77.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{75.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{75.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{74.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{62.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{46.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies on all MNIST networks. Adv. Training ~\citep{madry2017towards}, Bounded ~\citep{kolter2017provable}, IBP ~\citep{gowal2019effectiveness}, ReLU Stability ~\citep{xiao2019training}. For the medium CNN architecture, accuracies are found over 20 points.}
    \label{tab:mnist_full}
  %
\end{table}%



\begin{table}[htbp]
  \centering
  \adjustbox{max width = \textwidth}{
                    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
    Normal &       & 141.1 & 61.5\% & 22.0\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 1062.8 & 58.0\% & 24.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{5}[2]{*}{$\epsilon=2/255$} & 51203.7 & 57.5\% & 24.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 22351.6 & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 394.8 & 47.0\% & 37.5\% & 22.0\% & 3.5\% & 3.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 409.4 & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{394.5} & \cellcolor[rgb]{ .851,  .851,  .851}45.0\% & \cellcolor[rgb]{ .851,  .851,  .851}40.0\% & \cellcolor[rgb]{ .851,  .851,  .851}34.0\% & \cellcolor[rgb]{ .851,  .851,  .851}25.5\% & \cellcolor[rgb]{ .851,  .851,  .851}24.0\% & \cellcolor[rgb]{ .851,  .851,  .851}2.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% \\
    \midrule
    Adv. Training & \multirow{5}[2]{*}{$\epsilon=8/255$} & 51893.6 & \textbf{60.5\%} & 25.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 21918.7 & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 3.5\% & 3.5\% & 3.5\% \\
    IBP   &       & 410.0 & 37.5\% & 35.0\% & 32.5\% & 20.0\% & 17.5\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 396.1 & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}409.7 & \cellcolor[rgb]{ .851,  .851,  .851}45.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{45.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{43.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{40.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{39.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{28.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{22.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{19.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{15.0\%} \\
    \midrule
    \multicolumn{12}{c}{Medium CNN CIFAR, 7 layer} \\
    \midrule
    Normal &       & 1778.3 & 50.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=2/255$} & 6613.4 & \textbf{50.0\%} & \textbf{35.0\%} & 20.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}5770.2 & \cellcolor[rgb]{ .851,  .851,  .851}35.0\% & \cellcolor[rgb]{ .851,  .851,  .851}25.0\% & \cellcolor[rgb]{ .851,  .851,  .851}15.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=8/255$} & 6598.8 & 20.0\% & 15.0\% & 15.0\% & 10.0\% & 10.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{5762.2} & \cellcolor[rgb]{ .851,  .851,  .851}25.0\% & \cellcolor[rgb]{ .851,  .851,  .851}25.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{25.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{25.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{25.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{25.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{20.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{10.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{10.0\%} \\
    \midrule
    \multicolumn{12}{c}{Pooling CNN CIFAR, 5 layer} \\
    \midrule
    Normal &       & 1164.9 & 65.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 828.8 & 59.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=2/255$} & 4112.8 & 52.0\% & 24.0\% & 16.0\% & 6.0\% & 4.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 1682.6 & \textbf{60.5\%} & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}4091.4 & \cellcolor[rgb]{ .851,  .851,  .851}50.5\% & \cellcolor[rgb]{ .851,  .851,  .851}30.5\% & \cellcolor[rgb]{ .851,  .851,  .851}23.5\% & \cellcolor[rgb]{ .851,  .851,  .851}11.0\% & \cellcolor[rgb]{ .851,  .851,  .851}8.0\% & \cellcolor[rgb]{ .851,  .851,  .851}1.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=8/255$} & 4015.1 & 43.0\% & 15.5\% & 8.5\% & 3.0\% & 3.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{1676.9} & 58.5\% & 8.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}2899.5 & \cellcolor[rgb]{ .851,  .851,  .851}40.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{32.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{30.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{24.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{23.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{5.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{0.5\%} \\
    \midrule
    \multicolumn{12}{c}{1-Resnet CNN CIFAR, 4 layer} \\
    \midrule
    Normal &       & 1153.7 & 52.5\% & 4.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 847.3 & 58.0\% & 3.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=2/255$} & 3700.3 & \textbf{48.5\%} & 8.0\% & 6.0\% & 2.0\% & 2.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{1592.6} & 37.5\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}3393.9 & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{48.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{9.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{8.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}1.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=8/255$} & 3421.6 & 42.5\% & 2.5\% & 2.0\% & 1.0\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 1594.4 & 40.0\% & 1.0\% & 1.0\% & 1.0\% & 1.0\% & 1.0\% & 0.5\% & 0.5\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}3531.5 & \cellcolor[rgb]{ .851,  .851,  .851}35.0\% & \cellcolor[rgb]{ .851,  .851,  .851}4.0\% & \cellcolor[rgb]{ .851,  .851,  .851}4.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{3.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{3.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{3.5\%} \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies on all CIFAR networks. Adv. Training ~\citep{madry2017towards}, Bounded ~\citep{kolter2017provable}, IBP ~\citep{gowal2019effectiveness}, ReLU Stability ~\citep{xiao2019training}. For the mediun CNN architecture, accuracies are found over 20 points.}
  \label{tab:cifar_full}%
\end{table}%


\begin{table}[htbp]
  \centering
  \adjustbox{max width = \textwidth}{
    \begin{tabular}{llrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
    \textbf{Double Margin} & $\epsilon=0.2$ & 518.8 & \cellcolor[rgb]{ .851,  .851,  .851}93.44\% & \cellcolor[rgb]{ .851,  .851,  .851}93.15\% & \cellcolor[rgb]{ .851,  .851,  .851}92.61\% & \cellcolor[rgb]{ .851,  .851,  .851}92.06\% & \cellcolor[rgb]{ .851,  .851,  .851}91.30\% & \cellcolor[rgb]{ .851,  .851,  .851}89.63\% & \cellcolor[rgb]{ .851,  .851,  .851}78.55\% & \cellcolor[rgb]{ .851,  .851,  .851}0.00\% & \cellcolor[rgb]{ .851,  .851,  .851}0.00\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
    \textbf{Double Margin} & $\epsilon=8/255$ & 409.7 & \cellcolor[rgb]{ .851,  .851,  .851}43.00\% & \cellcolor[rgb]{ .851,  .851,  .851}41.71\% & \cellcolor[rgb]{ .851,  .851,  .851}40.58\% & \cellcolor[rgb]{ .851,  .851,  .851}37.72\% & \cellcolor[rgb]{ .851,  .851,  .851}37.25\% & \cellcolor[rgb]{ .851,  .851,  .851}28.44\% & \cellcolor[rgb]{ .851,  .851,  .851}22.39\% & \cellcolor[rgb]{ .851,  .851,  .851}19.06\% & \cellcolor[rgb]{ .851,  .851,  .851}16.35\% \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies computed on the entire test set.}
  \label{tab:full_test}%
\end{table}%


\begin{table}[htbp]
  \centering
  \adjustbox{max width = \textwidth}{
    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Medium CNN MNIST, 7 layer} \\
    \midrule
    Normal &       & 387.4 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[1]{*}{$\epsilon=0.1$} & 1553.6 & 98.5\% & 98.5\% & 98.5\% & 98.5\% & 97.5\% & 96.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1360.4 & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.0\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[0]{*}{$\epsilon=0.2$} & 1553.2 & 98.5\% & 98.5\% & 98.5\% & 98.0\% & 98.0\% & 97.0\% & 94.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1360.6 & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.0\% & \cellcolor[rgb]{ .851,  .851,  .851}93.5\% & \cellcolor[rgb]{ .851,  .851,  .851}89.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[1]{*}{$\epsilon=0.3$} & 1550.6 & 97.5\% & 97.5\% & 97.5\% & 97.5\% & 96.5\% & 95.5\% & 94.0\% & 90.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}1362.3 & \cellcolor[rgb]{ .851,  .851,  .851}90.5\% & \cellcolor[rgb]{ .851,  .851,  .851}90.5\% & \cellcolor[rgb]{ .851,  .851,  .851}88.5\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}87.0\% & \cellcolor[rgb]{ .851,  .851,  .851}83.5\% & \cellcolor[rgb]{ .851,  .851,  .851}79.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{12}{c}{Large CNN MNIST, 7 layer} \\
    \midrule
    Normal &       & 930.6 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[0]{*}{$\epsilon=0.1$} & 4162.8 & 98.0\% & 98.0\% & 98.0\% & 98.0\% & 97.0\% & 95.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}3742.5 & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}98.5\% & \cellcolor[rgb]{ .851,  .851,  .851}98.0\% & \cellcolor[rgb]{ .851,  .851,  .851}98.0\% & \cellcolor[rgb]{ .851,  .851,  .851}98.0\% & \cellcolor[rgb]{ .851,  .851,  .851}97.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[0]{*}{$\epsilon=0.2$} & 4162.3 & 98.5\% & 98.5\% & 98.5\% & 98.5\% & 97.5\% & 97.5\% & 93.5\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}3740.2 & \cellcolor[rgb]{ .851,  .851,  .851}97.5\% & \cellcolor[rgb]{ .851,  .851,  .851}97.0\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}96.5\% & \cellcolor[rgb]{ .851,  .851,  .851}95.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[1]{*}{$\epsilon=0.3$} & 4161.4 & 98.5\% & 98.0\% & 97.5\% & 97.5\% & 97.5\% & 97.5\% & 94.5\% & 91.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}3739.2 & \cellcolor[rgb]{ .851,  .851,  .851}93.0\% & \cellcolor[rgb]{ .851,  .851,  .851}93.0\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}92.0\% & \cellcolor[rgb]{ .851,  .851,  .851}91.0\% & \cellcolor[rgb]{ .851,  .851,  .851}84.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Medium CNN CIFAR, 7 layer} \\
    \midrule
    Normal &       & 1778.3 & 61.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[0]{*}{$\epsilon=2/255$} & 6613.4 & 45.5\% & 36.5\% & 27.0\% & 11.0\% & 9.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}5770.2 & \cellcolor[rgb]{ .851,  .851,  .851}45.0\% & \cellcolor[rgb]{ .851,  .851,  .851}37.0\% & \cellcolor[rgb]{ .851,  .851,  .851}24.5\% & \cellcolor[rgb]{ .851,  .851,  .851}10.5\% & \cellcolor[rgb]{ .851,  .851,  .851}8.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[1]{*}{$\epsilon=8/255$} & 6598.8 & 24.5\% & 24.5\% & 23.0\% & 21.5\% & 21.5\% & 18.5\% & 13.5\% & 12.0\% & 10.5\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}5762.2 & \cellcolor[rgb]{ .851,  .851,  .851}33.5\% & \cellcolor[rgb]{ .851,  .851,  .851}33.0\% & \cellcolor[rgb]{ .851,  .851,  .851}32.5\% & \cellcolor[rgb]{ .851,  .851,  .851}31.5\% & \cellcolor[rgb]{ .851,  .851,  .851}31.5\% & \cellcolor[rgb]{ .851,  .851,  .851}25.0\% & \cellcolor[rgb]{ .851,  .851,  .851}18.5\% & \cellcolor[rgb]{ .851,  .851,  .851}16.0\% & \cellcolor[rgb]{ .851,  .851,  .851}13.5\% \\
    \midrule
    \multicolumn{12}{c}{Large CNN CIFAR, 7 layer} \\
    \midrule
    Normal &       & 4020.6 & 65.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[1]{*}{$\epsilon=2/255$} & 17260.8 & 45.5\% & 33.5\% & 23.5\% & 10.0\% & 8.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}15141.5 & \cellcolor[rgb]{ .851,  .851,  .851}43.5\% & \cellcolor[rgb]{ .851,  .851,  .851}33.0\% & \cellcolor[rgb]{ .851,  .851,  .851}25.5\% & \cellcolor[rgb]{ .851,  .851,  .851}9.5\% & \cellcolor[rgb]{ .851,  .851,  .851}9.0\% & \cellcolor[rgb]{ .851,  .851,  .851}2.0\% & \cellcolor[rgb]{ .851,  .851,  .851}1.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=8/255$} & 17262.3 & 27.0\% & 27.0\% & 26.5\% & 25.0\% & 25.0\% & 23.5\% & 23.0\% & 22.5\% & 21.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}15131.7 & \cellcolor[rgb]{ .851,  .851,  .851}16.5\% & \cellcolor[rgb]{ .851,  .851,  .851}15.5\% & \cellcolor[rgb]{ .851,  .851,  .851}15.0\% & \cellcolor[rgb]{ .851,  .851,  .851}15.0\% & \cellcolor[rgb]{ .851,  .851,  .851}15.0\% & \cellcolor[rgb]{ .851,  .851,  .851}14.5\% & \cellcolor[rgb]{ .851,  .851,  .851}14.5\% & \cellcolor[rgb]{ .851,  .851,  .851}14.5\% & \cellcolor[rgb]{ .851,  .851,  .851}14.5\% \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Certified accuracies for large and medium CNN models computed using IBP~\citep{gowal2019effectiveness}.}
  \label{tab:ibp_cert}%
\end{table}%

==> Tab/tab_main.tex <==
\begin{table}[thbp]
    %\vspace*{-0.1in}
  \centering
   \adjustbox{max width = 0.95\textwidth}{
    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method (200 points)}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
    Normal &       & 185.7 & 98.5\% & 9.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 626.3 & 99.5\% & 81.0\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.3$} & 8760.5 & \textbf{99.5\%} & \textbf{98.5\%} & 91.5\% & 38.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27966.8 & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 29.5\% & 28.5\% & 25.0\% & 0.0\% \\
    IBP   &       & 611.2 & 95.5\% & 95.5\% & \textbf{95.5\%} & \textbf{90.5\%} & 76.5\% & 39.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 595.8 & 94.0\% & 90.0\% & 65.0\% & 23.0\% & 5.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 686.5 & 95.0\% & 88.0\% & 53.5\% & 13.5\% & 3.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9657.1 & 90.0\% & 86.5\% & 70.5\% & 55.0\% & 30.5\% & 13.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textcolor{our_methods}{\textbf{Double Margin}} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{520.0} & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.0\% & \cellcolor[rgb]{ .851,  .851,  .851}88.5\% & \cellcolor[rgb]{ .851,  .851,  .851}88.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}86.5\% & \cellcolor[rgb]{ .851,  .851,  .851}80.0\% & \cellcolor[rgb]{ .851,  .851,  .851}66.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textcolor{our_methods}{\textbf{Double Margin +L1}} &       & \cellcolor[rgb]{ .851,  .851,  .851}547.1 & \cellcolor[rgb]{ .851,  .851,  .851}91.0\% & \cellcolor[rgb]{ .851,  .851,  .851}90.5\% & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{89.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{87.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{83.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{68.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method (200 points)}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$2/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$7/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$9/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
    Normal &       & 141.1 & 61.5\% & 22.0\% & 1.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 1062.8 & 58.0\% & 24.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{5}[2]{*}{$\epsilon=8/255$} & 51893.6 & \textbf{60.5\%} & 25.0\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 21918.7 & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 4.0\% & 3.5\% & 3.5\% & 3.5\% \\
    IBP   &       & 410.0 & 37.5\% & 35.0\% & 32.5\% & 20.0\% & 17.5\% & 2.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{396.1} & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% & 12.0\% \\
    \textcolor{our_methods}{\textbf{Double Margin}} &       & \cellcolor[rgb]{ .851,  .851,  .851}409.7 & \cellcolor[rgb]{ .851,  .851,  .851}45.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{45.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{43.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{40.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{39.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{28.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{22.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{19.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{15.0\%} \\
    \midrule
    \multicolumn{12}{c}{Pooling CNN CIFAR, 5 layer} \\
    \midrule
    Normal &       & 1164.9 & 65.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 828.8 & 59.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{3}[2]{*}{$\epsilon=8/255$} & 4015.1 & 43.0\% & 15.5\% & 8.5\% & 3.0\% & 3.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{1676.9} & \textbf{58.5\%} & 8.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textcolor{our_methods}{\textbf{Double Margin}} &       & \cellcolor[rgb]{ .851,  .851,  .851}2899.5 & \cellcolor[rgb]{ .851,  .851,  .851}40.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{32.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{30.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{24.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{23.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{5.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{1.0\%}& \cellcolor[rgb]{ .851,  .851,  .851}\textbf{0.5\%} \\
    \midrule
    \multicolumn{12}{c}{Pureconv CNN GTSRB, 4 layer} \\
    \midrule
    Normal &       & 119.6 & 92.0\% & 77.5\% & 57.5\% & 37.0\% & 35.0\% & 6.5\% & 1.0\% & 0.0\% & 0.0\% \\
    \midrule
    IBP   & \multirow{2}[2]{*}{$\epsilon=8/255$} & 287.7 & 64.0\% & 63.0\% & 62.0\% & 58.5\% & 57.0\% & 44.5\% & 31.5\% & 26.0\% & 22.0\% \\
    \textcolor{our_methods}{\textbf{Double Margin}} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{283.1} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{68.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{67.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{67.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{65.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{64.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{58.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{52.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{50.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{45.5\%} \\
    \midrule
    \end{tabular}%
    }
    
    \adjustbox{max width = 0.95\textwidth}{
    \begin{tabular}{llrrrrrr}
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method (1000 points) }} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
TRADES & \multirow{7}[1]{*}{$\epsilon=0.3$}          &   8264.6       &   \textbf{99.5 (0.7)\%}       &   0.0 (0.0)\%    &   0.0 (0.0)\%    &   0.0 (0.0)\%    &   0.0 (0.0)\%    \\
IBP    &          &   611.2       &     96.3 (1.7)\%     &  92.2 (2.5)\%     &  46.5 (5.1)\%     &  0.0 (0.0)\%     &  0.0 (0.0)\%     \\ 
IBP *     &       &  460.9      &     96.7 (1.4)\%     &  90.3 (2.6)\%     &  39.3 (4.6)\%     &  0.0 (0.0)\%     &  0.0 (0.0)\%     \\ 
\textcolor{our_methods}{DM Variation 1}  &     &   \textbf{273.3}       &    94.0 (2.1)\%      &   \textbf{92.7 (2.5)\%}    &   \textbf{90.1 (3.0)\%}    &   78.0 (3.9)\%    &  33.1 (4.7)\%     \\ 
\textcolor{our_methods}{DM Variation 2}   &    &   589.6       &    90.1 (2.5)\%      &  88.9 (3.1)\%     &  86.5 (3.2)\%     &  \textbf{79.3 (3.7)\%}     &   59.0 (5.0)\%    \\ 
\textcolor{our_methods}{\textbf{Double Margin}} &  &  \cellcolor[rgb]{ .851,  .851,  .851}520.0        &    \cellcolor[rgb]{ .851,  .851,  .851}88.2 (2.6)\%      &  \cellcolor[rgb]{ .851,  .851,  .851} 86.7 (3.1)\%    &  \cellcolor[rgb]{ .851,  .851,  .851} 84.6 (3.4)\%    &  \cellcolor[rgb]{ .851,  .851,  .851}76.2 (3.9)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{61.9 (4.6)\%}     \\ 

\textcolor{our_methods}{\textbf{Double Margin} *}  &   &  \cellcolor[rgb]{ .851,  .851,  .851} 415.3      &   \cellcolor[rgb]{ .851,  .851,  .851} 91.1 (2.6)\%      &   \cellcolor[rgb]{ .851,  .851,  .851}90.1 (2.9)\%    &\cellcolor[rgb]{ .851,  .851,  .851}  87.6 (3.2)\%     &   \cellcolor[rgb]{ .851,  .851,  .851}78.4 (3.9)\%    &  \cellcolor[rgb]{ .851,  .851,  .851} 60.4 (4.7)\%    \\ 
\midrule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method (500 points)}} &   & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$1/255$}} &  \multicolumn{1}{c}{\multirow{2}[2]{*}{$3/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$5/255$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$8/255$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &    \\
    \midrule
\multicolumn{7}{c}{Small CNN CIFAR, 4 layer} \\
    \midrule
TRADES   & \multirow{5}[1]{*}{$\epsilon=8/255$}    &   56391.6       &    \textbf{62.2 (4.4)\%}     &  7.2 (2.5)\%    &  0.0 (0.0)\%     &  0.0 (0.0)\%    &   0.0 (0.0)\%   \\ 
IBP   &        &   2446.6       &    38.0 (4.2)\%      &  32.8 (4.0)\%     &  14.6 (3.1)\%     &   6.0 (2.2)\%    &   1.2 (0.8)\%    \\ 
\textcolor{our_methods}{DM Variation 1} &     &   \textbf{1475.8}       &     45.0 (5.1)\%     & \textbf{41.0 (3.8)\%}      &   33.8 (4.4)\%    &   22.8 (3.9)\%    &  10.4 (2.6)\%     \\
\textcolor{our_methods}{DM Variation 2}  &   &   3062.8       &   43.0 (4.6)\%       &  40.6 (4.2)\%     &  \textbf{34.2} (4.0)\%     &  27.0 (4.1)\%     &  18.2 (3.2)\%     \\ 
\textcolor{our_methods}{\textbf{Double Margin}} &  & \cellcolor[rgb]{ .851,  .851,  .851}2198.7       & \cellcolor[rgb]{ .851,  .851,  .851}  43.2 (4.0)\%       & \cellcolor[rgb]{ .851,  .851,  .851}40.4 (4.6)\%      &\cellcolor[rgb]{ .851,  .851,  .851}  32.8 (4.4)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{28.6 (4.4)\%}     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{19.8 (3.5)\%}     \\
\midrule
\multicolumn{7}{c}{Pureconv CNN GTSRB, 4 layer} \\
    \midrule
MMR (4 epochs)   &  \multirow{5}[1]{*}{$\epsilon=8/255$} &    85377.2      &    \textbf{88.2 (2.8)\%}      &    53.6 (4.0)\%   &  18.2 (3.7)\%     &   4.2 (1.8)\%    &   0.0 (0.0)\%    \\ 
IBP & &  287.7       &  71.8 (3.9)\%        &  68.0 (4.3)\%     &  60.8 (4.3)\%     &  47.6 (4.7)\%     &  28.2 (3.5)\%     \\ 
IBP *  &       &  266.6     &    78.0 (3.7)\%      &   \textbf{74.8 (3.7)\%}    &   62.2 (4.3)\%    &  45.6 (4.7)\%     &   26.8 (3.5)\%    \\ 
 \textcolor{our_methods}{\textbf{Double Margin}} & & \cellcolor[rgb]{ .851,  .851,  .851}283.1        &   \cellcolor[rgb]{ .851,  .851,  .851} 67.8 (4.4)\%      &  \cellcolor[rgb]{ .851,  .851,  .851}66.8 (4.3)\%     & \cellcolor[rgb]{ .851,  .851,  .851} 61.4 (4.3)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}56.4 (4.7)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{48.2 (4.5)\%}     \\ 
\textcolor{our_methods}{\textbf{Double Margin} *} &  &  \cellcolor[rgb]{ .851,  .851,  .851}\textbf{258.1}      &    \cellcolor[rgb]{ .851,  .851,  .851} 75.6 (3.9)\%     &  \cellcolor[rgb]{ .851,  .851,  .851}73.8 (4.2)\%      & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{65.0 (4.5)\%}     &  \cellcolor[rgb]{ .851,  .851,  .851} \textbf{57.2 (4.4)\%}    & \cellcolor[rgb]{ .851,  .851,  .851} 46.4 (4.4)\%     \\ 
\bottomrule
\end{tabular}
    }
    \caption{CNN-Cert certified accuracies and training times. std in ($\cdot$). * denotes a different setting of regularization parameter $\lam$, decreased from $\frac{1}{2}$ to $\frac{1}{4}$. MMR is trained for 4 epochs due to its long training time. Our methods or variants are in \textcolor{our_methods}{blue}.}
\end{table}%

==> Tab/tab_miniplace_relu.tex <==


%% Miniplace ReLU Full table

\begin{table}[htbp]
  \centering
    \begin{tabular}{rlrrrrrrrrrr}
    \toprule
    \multicolumn{1}{l}{Network} & Method & \multicolumn{1}{l}{Runtime} & \multicolumn{1}{l}{$\epsilon=0$} &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Large CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & ReLU Stabilty $\epsilon = 1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Pooling CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & ReLU Stabilty $\epsilon = 1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Resnet CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & ReLU Stabilty $\epsilon = 1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    \caption{MiniPlaces ReLU Table}
  %
\end{table}%

==> Tab/tab_miniplace_tanh.tex <==



%% Miniplace tanh full table

\begin{table}[htbp]
  \centering
    \begin{tabular}{rlrrrrrrrrrr}
    \toprule
    \multicolumn{1}{l}{Network} & Method & \multicolumn{1}{l}{Runtime} & \multicolumn{1}{l}{$\epsilon=0$} &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Large CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Pooling CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Resnet CNN MiniPlaces} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon =  1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =1/255$ &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    \caption{MiniPlaces Tanh Table}
  %
\end{table}%


==> Tab/tab_mnist_relu.tex <==



%% MNIST ReLU partial table: full table is in tab_full.tex

\begin{table}[thbp]
    \vspace*{-0.1in}
  \centering
   \adjustbox{max width = 1\textwidth}{
    \begin{tabular}{lcrrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} &       & \multicolumn{1}{l}{Training} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$\epsilon_{cert}=0$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.01$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.03$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.05$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.07$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.10$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.20$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.30$}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{$0.40$}} \\
          &       & \multicolumn{1}{l}{Time (sec)} &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{12}{c}{Small CNN MNIST, 4 layer} \\
    \midrule
    Normal &       & 185.7 & 98.5\% & 9.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 626.3 & 99.5\% & 81.0\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.2$} & 8786.8 & 99.0\% & \textbf{98.5\%} & 91.0\% & 38.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27999.5 & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 77.5\% & 75.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 614.0 & 97.5\% & 97.5\% & \textbf{97.0\%} & \textbf{96.5\%} & \textbf{96.0\%} & 78.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 592.6 & 95.0\% & 90.0\% & 59.0\% & 12.5\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 684.8 & 95.0\% & 89.5\% & 55.5\% & 10.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9669.4 & 93.0\% & 92.0\% & 86.5\% & 80.0\% & 63.5\% & 46.0\% & 3.5\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{518.8} & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.0\% & \cellcolor[rgb]{ .851,  .851,  .851}93.0\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}92.5\% & \cellcolor[rgb]{ .851,  .851,  .851}81.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textbf{Double Margin +L1} &       & \cellcolor[rgb]{ .851,  .851,  .851}546.1 & \cellcolor[rgb]{ .851,  .851,  .851}95.5\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}95.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{93.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}82.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    Adv. Training & \multirow{8}[2]{*}{$\epsilon=0.3$} & 8760.5 & \textbf{99.5\%} & \textbf{98.5\%} & 91.5\% & 38.5\% & 1.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Bounded &       & 27966.8 & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 30.0\% & 29.5\% & 28.5\% & 25.0\% & 0.0\% \\
    IBP   &       & 611.2 & 95.5\% & 95.5\% & 95.5\% & 90.5\% & 76.5\% & 39.5\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & 595.8 & 94.0\% & 90.0\% & 65.0\% & 23.0\% & 5.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    L1+RS+Pruning &       & 686.5 & 95.0\% & 88.0\% & 53.5\% & 13.5\% & 3.0\% & 0.5\% & 0.0\% & 0.0\% & 0.0\% \\
    Adv+RS+Pruning &       & 9657.1 & 90.0\% & 86.5\% & 70.5\% & 55.0\% & 30.5\% & 13.5\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}520.0 & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.0\% & \cellcolor[rgb]{ .851,  .851,  .851}88.5\% & \cellcolor[rgb]{ .851,  .851,  .851}88.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}86.5\% & \cellcolor[rgb]{ .851,  .851,  .851}80.0\% & \cellcolor[rgb]{ .851,  .851,  .851}66.5\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \textbf{Double Margin +L1} &       & \cellcolor[rgb]{ .851,  .851,  .851}547.1 & \cellcolor[rgb]{ .851,  .851,  .851}91.0\% & \cellcolor[rgb]{ .851,  .851,  .851}90.5\% & \cellcolor[rgb]{ .851,  .851,  .851}90.0\% & \cellcolor[rgb]{ .851,  .851,  .851}89.5\% & \cellcolor[rgb]{ .851,  .851,  .851}89.0\% & \cellcolor[rgb]{ .851,  .851,  .851}87.5\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{83.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{68.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \midrule
    \multicolumn{12}{c}{Pooling CNN MNIST, 5 layer} \\
    \midrule
    Normal &       & 226.0 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    Weight Regularization &       & 145.1 & 99.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \midrule
    Adv. Training & \multirow{4}[2]{*}{$\epsilon=0.2$} & 7573.4 & \textbf{99.5\%} & \textbf{98.5\%} & 16.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    IBP   &       & 1082.8 & 96.0\% & 78.0\% & 63.5\% & 51.0\% & 39.0\% & 20.0\% & 0.0\% & 0.0\% & 0.0\% \\
    ReLU Stabilty &       & \textbf{336.7} & 97.0\% & 90.0\% & 4.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
    \textbf{Double Margin} &       & \cellcolor[rgb]{ .851,  .851,  .851}680.5 & \cellcolor[rgb]{ .851,  .851,  .851}94.5\% & \cellcolor[rgb]{ .851,  .851,  .851}94.0\% & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{93.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{91.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{89.0\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{82.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}\textbf{4.5\%} & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% & \cellcolor[rgb]{ .851,  .851,  .851}0.0\% \\
    \bottomrule
    \end{tabular}%
    }
    \caption{CNN-Cert certified accuracies on MNIST networks}
    \label{tab:mnist_relu}
\end{table}%




==> Tab/tab_mnist_tanh.tex <==

%% mnist tanh full table

\begin{table}[htbp]
  \centering
    \begin{tabular}{rlrrrrrrrrrr}
    \toprule
    \multicolumn{1}{l}{Network} & Method & \multicolumn{1}{l}{Runtime} & \multicolumn{1}{l}{$\epsilon=0$} &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Small CNN MNIST} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .1$ &       &       &       &       &       &       &       &       &       &  \\
          & Bounded $\epsilon = .1$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .2$ &       &       &       &       &       &       &       &       &       &  \\
          & Bounded $\epsilon = .2$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .3$ &       &       &       &       &       &       &       &       &       &  \\
          & Bounded $\epsilon = .3$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Medium CNN MNIST} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .1$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .2$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & Adv. Training $\epsilon = .3$ &       &       &       &       &       &       &       &       &       &  \\
          & IBP $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Large CNN MNIST} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Pooling CNN MNIST} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{l}{Resnet CNN MNIST} & Normal &       &       &       &       &       &       &       &       &       &  \\
          & Weight Regularization &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.1$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.2$ &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{2-12}          & IBP $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
          & Double Margin $\epsilon =.3$ &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    \caption{MNIST Tanh Table}
  %
\end{table}%

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

